Towards Group-aware Search Success

Traditional measures of search success often overlook the varying information needs of different demographic groups. To address this gap, we introduce a novel metric, named Group-aware Search Success (GA-SS). GA-SS redefines search success to ensure that all demographic groups achieve satisfaction from search outcomes. We introduce a comprehensive mathematical framework to calculate GA-SS, incorporating both static and stochastic ranking policies and integrating user browsing models for a more accurate assessment. In addition, we have proposed Group-aware Most Popular Completion (gMPC) ranking model to account for demographic variances in user intent, aligning more closely with the diverse needs of all user groups. We empirically validate our metric and approach with two real-world datasets: one focusing on query auto-completion and the other on movie recommendations, where the results highlight the impact of stochasticity and the complex interplay among various search success metrics. Our findings advocate for a more inclusive approach in measuring search success, as well as inspiring future investigations into the quality of service of search.

==> 04-prelims.tex <==
\section{Preliminaries}
\label{sec:prelim}

Before we formally \HL{define the search success for achieving the quality-of-service fairness}, we go over some of the fundamental concepts in this section that have already been developed in existing literature that we build on in subsequent sections.

\subsection{Exposure and User Browsing Models}
\label{sec:prelim-user-model}

Simplified models of how users inspect and interact with retrieved results provide a useful tool for metric development~\citep{yilmaz2010expected, chuklin2013click} and for estimating relevance from historical logs of user behavior data~\citep{chuklin2015click}.
The user browsing model $\mu$ provides a mechanism to estimate the probability of exposure of an item $d$ in a retrieved ranked list of items $\sigma_q$ with respects to input query $q$.
For example, the user browsing model behind the rank-biased precision (RBP) metric~\citep{rbp} assumes that the probability of the exposure event $\epsilon_d$ for $d$ depends only on its rank $\rho_{\sigma_q}$ in $\sigma_q$ and decreases exponentially as we go down the ranked list.
\begin{align}
    %p_{\scaleto{RBP}{3pt}}(\epsilon|d,\sigma) &= (1 - \gamma) \cdot \gamma^{(\rho_{d,\sigma} - 1)}
    p(\epsilon_d|\sigma_q, \mu_{\scaleto{RBP}{3pt}}) &= \gamma^{\rho_{\sigma_q} - 1}
	\label{eqn:rbp-user-model},
\end{align}
where the $\gamma$ is the patience factor and controls how deep in the ranking the user is likely to browse, ``-1'' is to force the position starting from zero.


In this work, we employ the RBP user browsing model although other models can also be employed in its place.

\subsection{Stochastic Ranking and Expected Exposure}
\label{sec:prelim-expected-exposure}

\citet{diaz2020evaluating} define a stochastic ranking policy $\pi$ as a probability distribution over all permutations of items in the collection.
In the search scenario, let $\mathcal{D}$ be the collection of all items and $\mathcal{Q}$ the set of all input queries.
Now, given a stochastic ranking policy $\pi_q$ conditioned on input query $q \in \mathcal{Q}$, we can compute the expected value of the probability that an item $d \in \mathcal{D}$ is exposed to a searcher as below:
\begin{align}
    p(\epsilon_d|\pi_q) &= \mathbb{E}_{\sigma \sim \pi_q}\left[p(\epsilon_d|\sigma,\mu)\right].
	\label{eqn:expected-exposure}
\end{align}

Assuming the RBP user browsing model, we can further compute $p(\epsilon_d|\sigma,\mu)$ based on 
 Eq.~\ref{eqn:rbp-user-model}.
% Furthermore, for notational convenience, let $\mathsf{E} \in \mathbb{R}^{|\mathcal{Q}| \times |\mathcal{D}|}$ be the expected exposure matrix, such that $\mathsf{E}_{ij} = p(\epsilon_{\mathcal{D}_j}| \pi_{\mathcal{Q}_i})$.
% In the rest of this paper, we refer to the expected exposure $\mathsf{E}$ corresponding to a stochastic ranking policy $\pi$ as determined by a search system as \emph{system exposure}.
% Similarly, \emph{target exposure} is defined as the expected exposure $\mathsf{E}^*$ corresponding to an ideal stochastic ranking policy $\pi^*$, whose behavior may be dictated by some desirable principle, such as the \emph{equal expected exposure principle}~\citep{diaz2020evaluating}.
% The deviation of $\mathsf{E}$ from $\mathsf{E}^*$ gives us a quantitative measure of the suboptimality of the search system under consideration.
% Finally, we define \emph{random exposure} as the expected exposure $\mathsf{E}^\sim$ corresponding to a stochastic ranking policy $\pi^\sim$ which is defined by a uniformly random distribution over all permutations of items in the collection.





==> 99-ack.tex <==
\begin{acks}
Thank everyone!  \textbackslash(^-^)/
\end{acks}
